Dead ends and rationality of complete growth series

The complete growth series of a finitely generated group is given by $\sum_{n\ge 0} A_ns^n$, where $A_n$ is the sum of elements of length $n$ in the group semiring. We study the $\mathbb NG$-rationality and $\mathbb NG$-algebraicity of such series. We show that having dead ends of arbitrarily large depths is an obstruction to $\mathbb NG$-rationality. In the case of the $3$-dimensional Heisenberg group $H_3(\mathbb Z)$, we prove that the complete series is not $\mathbb NG$-algebraic for any generating set. Dead ends are also used to show that complete growth series of higher Heisenberg groups are not $\mathbb NG$-rational for specific generating sets. Using a more general version of this obstruction, we prove that complete growth series of some lamplighter groups are not $\mathbb NG$-rational either.

==> Source_files/tikz_cube.tex <==
\begin{tikzpicture}[scale=3.5]
    %%% Edit the following color
    
    \colorlet{colD}{Green}
    \colorlet{colLB}{red}
    \colorlet{colRB}{blue}
    \colorlet{colLF}{blue}
    \colorlet{colRF}{red}
    \colorlet{colU}{yellow}
    
    
	\coordinate (P) at (6,4.2); 
	\pgfmathsetmacro{\rati}{.9}
	\pgfmathsetmacro{\ninv}{.07}
	\pgfmathsetmacro{\midrat}{.5+.5*\rati}
	\pgfmathsetmacro{\almrat}{\ninv+(1-\ninv)*\rati}
	
	\coordinate (A1) at (0,0);
	\coordinate (A2) at (1,0);
	\coordinate (A3) at (1,1);
	\coordinate (A4) at (0,1);
	
	\coordinate (B1) at ($(P)!\rati!(A1)$);
	\coordinate (B2) at ($(P)!\rati!(A2)$);
	\coordinate (B3) at ($(P)!\rati!(A3)$);
	\coordinate (B4) at ($(P)!\rati!(A4)$);
    
    \coordinate (AB3) at ($(P)!\midrat!(A3)$);
    \coordinate (X) at ({1-\ninv},1);
    \coordinate (X1) at ($(P)!\midrat!(X)$);
    \coordinate (X2) at ($(P)!\rati!(X)$);
    \coordinate (Y) at (0,.5);
    \coordinate (Y1) at ($(P)!\almrat!(Y)$);
    \coordinate (Y2) at ($(P)!\rati!(Y)$);
    \coordinate (AB1) at ($(P)!\almrat!(A1)$);
    \coordinate (AB2) at ($(P)!{-.2+1.2*\rati}!(A1)$);
    
    \begin{scope}[thick]
    	\draw (A1) -- (A2) -- (A3) -- (A4) -- cycle;
    	\draw (B2) -- (B3) -- (B4);
    	\draw (A2) -- (B2);
    	\draw (A3) -- (B3);
    	\draw (A4) -- (B4);
    	
    	\draw[-latex] (A1) -- (1.15,0);
    	\node at (1.12,-.07) {$x$};
    	\draw[-latex] (A1) -- (0,1.15);
    	\node at (-.07,1.12) {$y$};
    \end{scope}
    
    %\begin{scope}[dotted, thick]
    \draw (B4) -- (B1) -- (B2);
    \draw (A1) -- (B1);
    \draw[-latex] (B1) -- (AB2);
    %\end{scope}
    
    \draw[ultra thick, red, rounded corners=1pt, decoration={markings, mark=at position 0.935 with {\arrow{latex}}}, postaction=decorate] (A1) -- (0.5,0) -- (0.5,\ninv) -- (1,\ninv) -- (A3) -- (AB3) -- (X1) -- (X2) -- (B4) -- (Y2) -- (Y1) -- (AB1) -- cycle;
    
    \draw[thick] (A4) -- (.99,1);
    
\end{tikzpicture}
